A Just and Comprehensive Strategy for Using NLP to Address Online Abuse

Online abusive behavior affects millions and the NLP community has attempted to mitigate this problem by developing technologies to detect abuse. However, current methods have largely focused on a narrow definition of abuse to detriment of victims who seek both validation and solutions. In this position paper, we argue that the community needs to make three substantive changes: (1) expanding our scope of problems to tackle both more subtle and more serious forms of abuse, (2) developing proactive technologies that counter or inhibit abuse before it harms, and (3) reframing our effort within a framework of justice to promote healthy communities.

==> old-text.tex <==

We argue that to achieve a just and productive online public space, NLP must develop language technologies along three fronts, under a banner of promoting  justice.
\begin{comment}
Intro summarizes the core problems we want to address
\begin{itemize}
    \item Lack of support for hard and serious challenges like the things addressed by heartmob.  The classification systems we used aren't design with comprehensiveness in mind, which leads to a false sense of progress and a lack of solutions to the many problems outside of those domains
    
    \item Current approaches ignore community norms.  Phrases that are offensive in one context may actually be positive and a sign of in-community bond.  The currently used datasets from Twitter and Wikipedia are poor models for general norms.  Probably want to say something about how the norms of marginalized communities are overlooked in our current solutions.
    
    \item The community has only focused on recognizing bad behavior with little thought of what constitutes good behavior.  The absence of toxic language and bad behavior is neither necessary or sufficient for a healthy community.  Methods that identify pro-social behaviors are needed to understand community health and behavior--and to ensure that when changes are made, positive behaviors are not affected.
    
    \item By the time we detect bad behavior, it might be too late to have an effect on the resulting outcomes.  We need methods that help both conversants and moderators \textit{before the situation gets bad}.
    
    \item The classification system itself isn't an end in itself and instead we need to pursue methods that lead to justice.  Roughly, we are optimizing our communities for the wrong thing.  A part of this will be on how sometimes emotion and bad behavior are necessary to achieve a constructive dialog and imposing unemotional language requirements may actually hinder us.  A second part will be thinking about models of justice within communities and how removing content (punitive justice) could be replaced with restorative justice methods (e.g., suggesting inoffensive paraphrases, which is an NLP technique)--the choice between whether punitive/restorative is applied could even be addressed using NLP (e.g., identify bad actors vs. those making correctable mistakes).
\end{itemize}
\end{comment}



\paragraph{Contributions}

NLP exists within a wider social ecosystem and the wide applicability of our tools can lead to significant positive impact and exposure.  This paper is an attempt to better contextualize the current NLP efforts within the broad space of social behavior and work on social system.

Another contribution is linking to work from psychology, social computing, etc., 

Meh... Something about how NLP currently largely exists within a vacuum and boils most problems down to those that are easily modeled when the larger world is far messier---and desperately needs the real problems addressed.  This paper introduces a series of methodological challenges that show how our current efforts should be better concentrated.

Some other contribution on how we reframe currently-missing areas of research as computational prediction tasks.  We point to high-impact area where new development in language technologies would be beneficial.

\daj{Second(?),} This paper proposes how the efforts to develop computational approaches can be redirected to new, more challenging NLP tasks that have concrete benefits of improving online platforms.


\begin{comment}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/big-picture-view.pdf}
    \caption{The big picture view of how we build just, successful online public spaces.  This emphasizes that abusive behavior detection is only a \textit{part} of the whole solution and that the current focus in abusive behavior is in practice only a small part of the space of abuse as well!}
    \label{fig:big-picture}
\end{figure*}
\end{comment}




\subsection{Nuanced predictions tasks over binary moderation decisions}
\ec{This is like the hint at a solution to the problem faced by current approaches to abuse detection---need to include norms in the decision-making process}

Scaling the idea of machine learning-based approaches to abuse detection up to groups interacting via an online community presents challenges, because of the social norms that emerge within a particular group. The members and moderators of those groups (communities) know those norms best, and expend considerable effort enforcing them.


\subsection{Contextual nature of abuse detection}
What communities consider to be abusive (or violations) are highly-contextual, and depend on the community's norms~\cite{chandrasekharan2018internet}. In other words, depending on the community that were are dealing with, the same type of behaviors could be either encouraged or discouraged.
In the end, the social norms of an online community are best understood by its members (and moderators), as the community defines which types of speech should be valued, or considered as norm violations (e.g., abusive). Instead of thinking of these competing norms as problematic, we could think the plurality of spaces and norms for public discussion as necessary for the creation of effective, inclusive public debate. Fraser \cite{Fraser1990-lu} explains that a single public space governed by dominant groups' rules about who can participate and how perpetuates group inequalities; without spaces of their own, subordinate groups cannot deliberate or organize to effectively advocate for themselves in the larger public conversation. Different communities with different norms are essential for a deliberation.  

When building tools to detect online abuse, it is important to take the community's norms into account. Given that different communities care about different sets of norm violations, the severity of infractions can vary given the context or the nature of the topic of discussion (e.g., sensitive topics around politics or mental health would require the moderators to be less tolerant of trolling or vitriol). 
These nuances are important to take into account, as platforms and researchers are doubling down on machine-learning approaches towards detecting abuse.

\ec{In addition to the community, author-level signals also affect what is perceived as abusive. e.g., in-group speech}



\paragraph{Evaluating the effectiveness of interventions}

\ec{How do we go about \textit{evaluating the effectiveness} of interventions in real-time? What is a ``successful'' intervention?} As external researchers, most of our focus is on tuning parameters for carefully constructed data sets. These may not be \emph{representative} of the actual settings under which our interventions are later applied. Also, what should we be optimizing for in these interventions? Performance gains in classifier accuracy may not be the only things we should care about when designing these interventions. Perhaps other metrics like quicker response time, and allowing the community to learn from their actions could also be key components to optimize for.

